PersisDroid: Android Performance Diagnosis via Anatomizing Asynchronous Executions

Android applications (apps) grow dramatically in recent years. Apps are user interface (UI) centric typically. Rapid UI responsiveness is key consideration to app developers. However, we still lack a handy tool for profiling app performance so as to diagnose performance problems. This paper presents PersisDroid, a tool specifically designed for this task. The key notion of PersisDroid is that the UI-triggered asynchronous executions also contribute to the UI performance, and hence its performance should be properly captured to facilitate performance diagnosis. However, Android allows tremendous ways to start the asynchronous executions, posing a great challenge to profiling such execution. This paper finds that they can be grouped into six categories. As a result, they can be tracked and profiled according to the specifics of each category with a dynamic instrumentation approach carefully tailored for Android. PersisDroid can then properly profile the asynchronous executions in task granularity, which equips it with low-overhead and high compatibility merits. Most importantly, the profiling data can greatly help the developers in detecting and locating performance anomalies. We code and open-source release PersisDroid. The tool is applied in diagnosing 20 open-source apps, and we find 11 of them contain potential performance problems, which shows its effectiveness in performance diagnosis for Android apps.

==> perf_test_discussion.tex <==
%\label{sec:perf_test_discussion}
%%根据我们找到的bug，提供给开发的建议
%\subsection{Tips for developers}
%\label{subsec:perf_test_tips}
%We have learned many kinds of bugs from the experiment.  Some tips for developers could be concluded from these bugs.
%
%%不要每次都用公共的线程池，公共线程池的资源也是有限的。如果真的要长时间运行，用自建线程池
%\subsubsection{\textbf{Use private pool instead of public one when necessary}}
%It is necessary defining your own thread pool instead of using a public pool like \texttt{AsyncTask.THREAD\_POOL\_EXECUTOR} in some case.
%%The thread pool is used either for directly executing tasks on or being called by \texttt{executeOnExecutor} of \texttt{AsyncTask}.  Current implementation of \texttt{AsyncTask.THREAD\_POOL\_EXECUTOR} has the thread pool size under $10$ in usual.  Therefore if too many \texttt{AsyncTask}s are put into the pool, it is easy to be used up.  
%We suggest defining your own thread pool especially for the case that the asynchronous execution takes a long time or the asynchronous execution will not update UI after finishes.  In the former case asynchronous execution would occupies a thread in the pool for long time.  In the later case, the asynchronous execution is not necessary to be implemented as \texttt{AsyncTask}.
%
%%设置合理的线程池大小，可以通过排队论方式推算，或者尝试几个参数并参考我们的工具调整
%\subsubsection{\textbf{Set reasonable pool size}}
%When using pool-based asynchronous execution, the developers should carefully set the pool size.
%%A small pool may increase the chance for an asynchronous execution to wait in the queue.  On the other hand a large pool may waste system resource if starving from works.
%%The developers could apply queuing models ({\em e.g.,} M/M/n model) for guessing a reasonable pool size.  Our tool could provide the service time (execution time) as a parameter of model.  The developers would decide the arrival time according to their experience.  
%A practical choice is that the developers could just try to set the pool size several times and run our tool.  After getting the reports for every run, a best choice among the previous settings could be found.
%
%%用第三方库时应当要注意使用说明
%\subsubsection{\textbf{Use third-party library carefully}}
%The developers should inspect the specification of third-party libraries carefully when utilizing them especially when there is potential asynchronous executions.
%%It is convenient to use third-party library.  However, the developers are usually not aware of the implementation details of the library.  The library may provide multiple implementations for an operation to suit different requirements and situations.  The implementations are separated by parameters passed when calling the function.
%The default setting of parameters might be only a moderate setting that meets most requirement.  If the developers did not read the specification carefully, they may set problematic parameters that does not fit into their requirement.  In which case, there would be potential performance bugs.
%
%%保证有效的相应，而不是progresscycle一直转圈圈等待。应当保持功能，或者至少可以回退
%\subsubsection{\textbf{Keep effective response}}
%Most developers know they should keep the screen response when an asynchronous execution is performed.
%%But they may sometime forget to make effective response.  In some cases, the developers simply display a progress bar/circle in the whole screen to show the execution is in progress.
%The user may get annoyed if a progress bar displays for long.  It could get even worse when the back button is disabled and the user could do nothing but wait for the execution.  It is acceptable that some operations could be delayed until an asynchronous execution done.  But at the same time the app should keep response to user interacts and better display some meaningful pages.
%
%%异步任务会占用资源，异步任务不在需要时要及时清除。（比如Activity都不在了，没有显示的地方应当清除）
%\subsubsection{\textbf{Cancel when no longer needed}}
%The developers often do not take care of cancelling the asynchronous executions when they are no longer needed.
%%For example, an asynchronous task which loads figures in an activity should be cancelled after the activity is hidden or destroyed.  Another example is when downloading a list of figures that would be displayed on the screen, the figures swiped out should be cancelled from downloading.
%All asynchronous execution requires resources including thread of pool-based executions, system resource like CPU, network and disk I/O, etc.  If long term asynchronous executions are not cancelled properly, thread pool may become exhausted or system resources may become shorted ({\em e.g.,} network becomes slow).
%
%%选择合适的异步执行方法。AsyncTask被建议仅用于短时间（几秒）的异步任务，长时间异步任务可能会引入bug。
%\subsubsection{\textbf{Use proper type of asynchronous execution}}
%There are different types of asynchronous executions, the unexperienced developers may not know which one is better to suit their requirement.  For example, \texttt{AsyncTask} is a class simplifying generic asynchronous execution.
%%Asynchronizer \cite{AndroidPerf:RefactorAsynctask} would refactor long concurrent works into \texttt{AsyncTask}s.
%But it is not a panacea.  Officially it is suggested that an asynctask should be used for short operations (a few seconds at the most) \cite{AndroidPerf:Asynctask}.  For long term operations,  it is common to introduce bugs in the design of \texttt{AsyncTask}.
%%For example, in the codes shown in Figure \ref{fig:perf_test_original_asynctask}, there is a bug in \texttt{RetrieveInfoTask} class.  It may take $20$ seconds to retrieve the data from Internet.  If during that time the activity is destroyed, however, the \texttt{RetrieveInfoTask} will run until it finishes.  When the \texttt{onPostExecute} is invoked, the text view no longer exists and the program would be crashed if the error is not catched.  Therefore it is not appropriate to use \texttt{AsyncTask} for network requests which may takes very long.  Developers then resort to \texttt{Loader} class.  However,
%As suggested in RoboSpice project \cite{AndroidPerf:RoboSpice}, \texttt{AsyncTask} has its limitation on performing network requests.  RoboSpice project \cite{AndroidPerf:RoboSpice} may be a better choice for this case.  The developers should better understand the features of different types of asynchronous executions and apply suitable one when needed.  Misusing of asynchronous executions could introduce performance bugs.

%\subsection{Discussions on the implementation}
%\subsubsection{Hooking methods of apks}
%Method hooking is the first step (pre-run step) of our testing framework.  When talking about hooking methods in app, the first idea is decompile and modify the apk file.  There are already several tools that could do the decompile/recompile like smali \cite{Android:smali} and apktool \cite{Android:apktool}.  However many apks would obfuscate the codes when release.  Most obfuscated codes could
%Therefore we resort to run time hijacking the framework code which is obfuscated.


%%我们工具的overhead，我们暂时不去优化，因为我们认为在测试中，这不是最重要的
%\subsection{Tool overhead}
%We leave the task of optimizing overhead of this tool for future work as we believe this is not a critical issue for the testing phase.  Moreover, our tool could be used for the initial performance test only.  That means our tool would find some suspicious asynchronous executions then the developers could do the method hooking themselves.
%
%%我们工具不能测同步任务中包含的性能问题
%\subsection{Limitation of our tool}
%\main thread is different from worker threads.  \main thread is not task-oriented.  It keeps running during the whole life of the app.  We do not test problems on \main thread. Therefore those performance issues caused by bad design of \main thread will not be detected by our tools.  As mentioned in Section \ref{sec:perf_test_perfproblems} several tools address and try to solve this problem.

